Mapping Firms' Locations in Technological Space: A Topological Analysis of Patent Statistics

Where do firms innovate? Mapping their locations and directions in technological space is challenging due to its high dimensionality. We propose a new method to characterize firms' inventive activities via topological data analysis (TDA) that represents high-dimensional data in a shape graph. Applying this method to 333 major firms' patents in 1976--2005 reveals substantial heterogeneity: some firms remain undifferentiated; others develop unique portfolios. Firms with unique trajectories, which we define and measure graph-theoretically as "flares" in the Mapper graph, perform better. This association is statistically and economically significant, and continues to hold after we control for portfolio size, firm survivorship, industry classification, and firm fixed effects. By contrast, existing techniques -- such as principal component analysis (PCA) and Jaffe's (1989) clustering method -- struggle to track these firm-level dynamics.

==> Tables/Table_EBIT_n20.tex <==
\begin{table}[tbh!!!!]
\caption{EBIT and Flares $\left( n=20\right) $}
\label{Table - EBIT (n = 20)}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(EBIT in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.536$ & $0.311$ & $-$ & $-$ &  & $1.928$
& $0.145$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.209)$ & $(0.270)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.209)$ & $(0.278)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $1.731$ & $0.000$ & $-$ & $-$ &  & $%
1.921$ & $-0.601$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.505)$ & $(0.538)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.449)$ & $(0.494)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.913$ & $1.731$ & $-$ & $-$ &  & $3.207$
& $0.459$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.672)$ & $(0.708)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.708)$ & $(0.703)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.056$ & $0.309$ &  & $-$
& $-$ & $1.330$ & $0.050$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.227)$ & 
$(0.061)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.237)$ & $%
(0.285) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $2.185$ & $0.206$ &  & $-$
& $-$ & $2.381$ & $0.524$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.512)$ & 
$(0.273)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.469)$ & $%
(0.507) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.209$ & $1.010$ &  & $-$
& $-$ & $2.217$ & $0.441$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.568)$ & 
$(0.540)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.545)$ & $%
(0.562) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $1.958$ & $0.877$ &  & $-$
& $-$ & $2.966$ & $0.636$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.568)$ & 
$(0.602)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.515)$ & $%
(0.580) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.778$ & $0.578$ &  & $-$
& $-$ & $2.860$ & $0.662$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.712)$ & 
$(0.606)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.515)$ & $%
(0.569) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.005$ & $1.255$ &  & $-$
& $-$ & $3.095$ & $0.687$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.606)$ & 
$(0.742)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.762)$ & $%
(0.781) $ \\ 

\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$
& $-$ & $1.282$ & $-1.382$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ & 
$\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.510)$ & $%
(1.438) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.462$ & $1.376$ &  & $-$
& $-$ & $5.128$ & $2.659$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.570)$ & 
$(0.660)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.510)$ & $%
(1.431) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $2.791$ & $1.834$ &  & $%
- $ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.114)$ & 
$(1.531)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 

\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.913$ & $0.939$
&  & $-$ & $-$ & $3.207$ & $0.811$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.652)$ & 
$(1.123)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.683)$ & $%
(0.716) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.373$ & $-$ & $2.106$ &  & $-$ & $%
0.624$ & $-$ & $0.544$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $(0.057)$ & $\left( -\right) $ & 
$(0.716)$ &  & $\left( -\right) $ & $(0.073)$ & $\left( -\right) $ & $%
(0.078) $ \\ 
\multicolumn{1}{l}{Constant} & $5.125$ & $3.627$ & $5.125$ & $3.884$ &  & $%
5.105$ & $1.999$ & $5.105$ & $2.396$ \\ 
\multicolumn{1}{l}{} & $(0.134)$ & $(0.261)$ & $(0.130)$ & $(0.273)$ &  & $%
(0.122)$ & $(0.378)$ & $(0.118)$ & $(0.405)$ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.233$ & $0.339$ & $0.279$ & $0.344$
&  & $0.280$ & $0.437$ & $0.328$ & $0.434$ \\ 
\multicolumn{1}{l}{Number of observations} & $262$ & $262$ & $262$ & $262$ & 
& $264$ & $264$ & $264$ & $264$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: The RHS variables are based on the topological characterization of patent statistics between 1976 and 2005. Standard errors are in parentheses.}
\end{minipage}
\end{center}
\end{table}

==> Tables/Table_EBIT_n20_with_sector_dummies.tex <==

\begin{table}[tbh]
\caption{EBIT (Earnings before Interest and Taxes) and Flares $\left( n=20\right) $}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(EBIT in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.583$ & $0.397$ & $-$ & $-$ &  & $1.939$
& $0.189$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.206)$ & $(0.263)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.205)$ & $(0.267)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $1.838$ & $0.135$ & $-$ & $-$ &  & $%
1.832$ & $-0.695$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.495)$ & $(0.527)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.442)$ & $(0.480)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.958$ & $1.784$ & $-$ & $-$ &  & $3.515$
& $0.799$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.707)$ & $(0.733)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.674)$ & $(0.664)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.076$ & $0.310$ &  & $-$
& $-$ & $1.305$ & $0.093$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.215)$ & 
$(0.262)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.227)$ & $(0.273)
$ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $2.351$ & $1.294$ &  & $-$
& $-$ & $2.492$ & $0.720$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.487)$ & 
$(0.517)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.449)$ & $(0.487)
$ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.698$ & $1.453$ &  & $-$
& $-$ & $2.443$ & $0.752$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.539)$ & 
$(0.580)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.525)$ & $(0.541)
$ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.047$ & $0.737$ &  & $-$
& $-$ & $3.156$ & $0.861$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.550)$ & 
$(0.595)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.496)$ & $(0.565)
$ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.825$ & $1.407$ &  & $-$
& $-$ & $2.859$ & $0.684$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.692)$ & 
$(0.728)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.501)$ & $(0.558)
$ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.434$ & $1.908$ &  & $-$
& $-$ & $3.428$ & $1.089$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.593)$ & 
$(0.653)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.722)$ & $(0.745)
$ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $1.896$ & $-0.667$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(-)$ & $(-)
$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.426)$ & $(1.361)$ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.653$ & $2.056$ &  & $-$
& $-$ & $3.672$ & 1.355 \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.513)$ & 
$(1.489)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.470)$ & $(1.390)
$ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.212$ & $1.509$ &  & $-
$ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.045)$ & 
$(1.064)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $4.050$ & $2.348$
&  & $-$ & $-$ & $3.548$ & $1.240$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.672)$ & 
$(0.737)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.647)$ & $(0.682)
$ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.360$ & $-$ & $0.276$ &  & $-$ & $%
0.612$ & $-$ & $0.516$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $(0.055)$ & $\left( -\right) $ & 
$(0.058)$ &  & $\left( -\right) $ & $(0.069)$ & $\left( -\right) $ & $(0.075)
$ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.301$ & $0.402$ & $0.369$ & $0.420$
&  & $0.355$ & $0.507$ & $0.407$ & $0.500$ \\ 
\multicolumn{1}{l}{Number of observations} & $262$ & $262$ & $262$ & $262$ & 
& $264$ & $264$ & $264$ & $264$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: Standard errors are in parentheses. S\&P economic sector dummies are included.}
\end{minipage}
\end{center}
\label{Table - EBIT (n = 20)}
\end{table}

==> Tables/Table_Mcap_n20.tex <==

\begin{table}[tbh!!!!]
\caption{Stock-Market Capitalization and Flares $\left( n=20\right) $}
\label{Table - Mcap (n = 20)}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.507$ & $0.150$ & $-$ & $-$ &  & $1.880$
& $-0.009$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.206)$ & $(0.260)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.206)$ & $(0.269)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.483$ & $0.527$ & $-$ & $-$ &  & $%
2.551$ & $-0.171$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.495)$ & $(0.520)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.443)$ & $(0.482)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.799$ & $1.338$ & $-$ & $-$ &  & $3.172$
& $0.205$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.687)$ & $(0.706)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.724)$ & $(0.705)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.187$ & $0.126$ &  & $-$
& $-$ & $1.505$ & $-0.006$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.226)$ & 
$(0.266)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.235)$ & $%
(0.276) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.678$ & $0.237$ &  & $-$
& $-$ & $1.853$ & $-0.215$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.469)$ & 
$(0.489)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.434)$ & $%
(0.458) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.447$ & $0.777$ &  & $-$
& $-$ & $2.228$ & $0.135$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.589)$ & 
$(0.605)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.564)$ & $%
(0.562) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.022$ & $0.291$ &  & $-$
& $-$ & $3.222$ & $0.469$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.589)$ & 
$(0.609)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.534)$ & $%
(0.577) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.884$ & $0.974$ &  & $-$
& $-$ & $2.953$ & $0.357$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.738)$ & 
$(0.747)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.534)$ & $%
(0.567) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.055$ & $1.011$ &  & $-$
& $-$ & $3.161$ & $0.316$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.628)$ & 
$(0.663)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.789)$ & $%
(0.781) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$
& $-$ & $1.218$ & $-1.930$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ & 
$\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.566)$ & $%
(1.447) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.040$ & $0.997$ &  & $-$
& $-$ & $4.790$ & $1.873$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.630)$ & 
$(1.550)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.566)$ & $%
(1.440) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.121$ & $0.794$ &  & $%
- $ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.157)$ & 
$(1.134)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.799$ & $1.528$
&  & $-$ & $-$ & $3.172$ & $0.341$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.676)$ & 
$(0.719)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.708)$ & $%
(0.716) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.423$ & $-$ & $0.391$ &  & $-$ & $%
0.678$ & $-$ & $0.647$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $(0.056)$ & $\left( -\right) $ & 
$(0.060)$ &  & $\left( -\right) $ & $(0.072)$ & $\left( -\right) $ & $%
(0.077) $ \\ 
\multicolumn{1}{l}{Constant} & $7.614$ & $5.896$ & $7.614$ & $6.029$ &  & $%
7.595$ & $4.206$ & $7.595$ & $4.360$ \\ 
\multicolumn{1}{l}{} & $(0.132)$ & $(0.257)$ & $(0.130)$ & $(0.271)$ &  & $%
(0.120)$ & $(0.374)$ & $(0.118)$ & $(0.397)$ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.233$ & $0.361$ & $0.257$ & $0.356$
&  & $0.280$ & $0.451$ & $0.310$ & $0.450$ \\ 
\multicolumn{1}{l}{Number of observations} & $284$ & $284$ & $284$ & $284$ & 
& $286$ & $286$ & $286$ & $286$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: The RHS variables are based on the topological characterization of patent statistics between 1976 and 2005. Standard errors are in parentheses.}
\end{minipage}
\end{center}
\end{table}


==> Tables/Table_Mcap_n20_with_sector_dummies.tex <==

\begin{table}[tbh!!!!]
\caption{Stock-Market Capitalization and Flares $\left( n=20\right) $}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Market capitalization in 2005)} \\ 
\cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.543$ & $0.241$ & $-$ & $-$ &  & $1.882$
& $0.062$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.202)$ & $(0.253)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.202)$ & $\left( 0.260\right) $ & $\left( -\right) $ & $%
\left( -\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.532$ & $0.627$ & $-$ & $-$ &  & $%
2.399$ & $-0.277$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.483)$ & $(0.507)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.436)$ & $\left( 0.473\right) $ & $\left( -\right) $ & $%
\left( -\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.895$ & $1.466$ & $-$ & $-$ &  & $3.458$
& $0.576$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.719)$ & $(0.730)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.691)$ & $\left( 0.674\right) $ & $\left( -\right) $ & $%
\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.188$ & $0.217$ &  & $-$
& $-$ & $1.448$ & $0.048$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.215)$ & 
$(0.255)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.225\right) $ & $\left( 0.266\right) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.805$ & $0.489$ &  & $-$
& $-$ & $1.957$ & $0.028$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.448)$ & 
$(0.470)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.416\right) $ & $\left( 0.443\right) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.819$ & $1.243$ &  & $-$
& $-$ & $2.331$ & $0.384$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.559)$ & 
$(0.582)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.543\right) $ & $\left( 0.544\right) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.148$ & $0.480$ &  & $-$
& $-$ & $3.462$ & $0.809$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.571)$ & 
$(0.599)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.514\right) $ & $\left( 0.567\right) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $3.052$ & $1.246$ &  & $-$
& $-$ & $2.935$ & $0.425$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.720)$ & 
$(0.735)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.519\right) $ & $\left( 0.560\right) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.320$ & $1.386$ &  & $-$
& $-$ & $3.434$ & $0.736$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.614)$ & 
$(0.654)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.749\right) $ & $\left( 0.751\right) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $1.548$ & $-1.406$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $\left( 1.478\right) $ & $\left( 1.377\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.478$ & $1.438$ &  & $-$
& $-$ & $3.180$ & $0.492$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.575)$ & 
$(1.511)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.526\right) $ & $\left( 1.410\right) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.472$ & $1.304$ &  & $-
$ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.087)$ & 
$(1.076)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.973$ & $1.805$
&  & $-$ & $-$ & $3.490$ & $0.822$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.698)$ & 
$(0.742)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.670\right) $ & $\left( 0.687\right) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.401$ & $-$ & $0.355$ &  & $-$ & $%
0.652$ & $-$ & $0.599$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $(0.054)$ & $\left( -\right) $ & 
$(0.057)$ &  & $\left( -\right) $ & $(0.069)$ & $\left( -\right) $ & $\left(
0.074\right) $ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.306$ & $0.424$ & $0.347$ & $0.428$
&  & $0.351$ & $0.509$ & $0.390$ & $0.508$ \\ 
\multicolumn{1}{l}{Number of observations} & $284$ & $284$ & $284$ & $284$ & 
& $286$ & $286$ & $286$ & $286$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: Standard errors are in parentheses. S\&P economic sector dummies are included.}
\end{minipage}
\end{center}
\label{Table - Mcap (n = 20)}
\end{table}

==> Tables/Table_Regressions_alt.tex <==
\begin{table}[tbh!!!!]
\caption{Flare Regressions Based on Alternative Distance Metrics}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccccc}
\hline \hline
LHS variable: & \multicolumn{3}{c}{Log(Revenue)} &  & \multicolumn{3}{c}{
Log(EBIT)} &  & \multicolumn{3}{c}{Log(Market value)} \\ 
\cline{2-4}\cline{3-4}\cline{6-8}\cline{10-12}
Distance metric: & Euclid & Correl & Min-c &  & Euclid & Correl & Min-c &  & 
Euclid & Correl & Min-c \\ 
& (1) & (2) & (3) &  & (4) & (5) & (6) &  & (7) & (8) & (9) \\ \hline
\multicolumn{1}{l}{Constant (= no flare)} & $6.07$ & $6.07$ & $6.05$ &  & $3.89
$ & $3.96$ & $3.86$ &  & $6.08$ & $6.17$ & $6.13$ \\ 
\multicolumn{1}{l}{} & $\left( 0.22\right) $ & $\left( 0.22\right) $ & $%
\left( 0.22\right) $ &  & $\left( 0.24\right) $ & $\left( 0.24\right) $ & $%
\left( 0.24\right) $ &  & $\left( 0.24\right) $ & $\left( 0.24\right) $ & $%
\left( 0.24\right) $ \\ 
\multicolumn{1}{l}{Flare length} & $0.31$ & $0.33$ & $0.28$ &  & $0.25$ & $%
0.31$ & $0.21$ &  & $0.17$ & $0.25$ & $0.19$ \\ 
\multicolumn{1}{l}{} & $\left( 0.08\right) $ & $\left( 0.08\right) $ & $%
\left( 0.08\right) $ &  & $\left( 0.08\right) $ & $\left( 0.08\right) $ & $%
\left( 0.08\right) $ &  & $\left( 0.08\right) $ & $\left( 0.08\right) $ & $%
\left( 0.08\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $1.04$ & $1.24$ & $1.99$ &  & $0.71$ & $%
1.15$ & $1.47$ &  & $0.16$ & $0.89$ & $1.11$ \\ 
\multicolumn{1}{l}{} & $\left( 1.02\right) $ & $\left( 0.73\right) $ & $%
\left( 0.74\right) $ &  & $\left( 1.08\right) $ & $\left( 0.77\right) $ & $%
\left( 0.78\right) $ &  & $\left( 1.11\right) $ & $\left( 0.79\right) $ & $%
\left( 0.79\right) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $0.28$ & $0.28$ & $0.29$ &  & $0.32$ & $%
0.30$ & $0.33$ &  & $0.38$ & $0.35$ & $0.36$ \\ 
\multicolumn{1}{l}{} & $\left( 0.04\right) $ & $\left( 0.22\right) $ & $%
\left( 0.04\right) $ &  & $\left( 0.05\right) $ & $\left( 0.05\right) $ & $%
\left( 0.05\right) $ &  & $\left( 0.05\right) $ & $\left( 0.05\right) $ & $%
\left( 0.05\right) $ \\ \hline
\multicolumn{1}{l}{$R^{2}$} & $.338$ & $.345$ & $.339$ &  & $.329$ & $.343$
& $.326$ &  & $.328$ & $.339$ & $.332$ \\ 
\multicolumn{1}{l}{Adjusted $R^{2}$} & $.332$ & $.339$ & $.333$ &  & $.322$
& $.336$ & $.320$ &  & $.322$ & $.333$ & $.326$ \\ 
\multicolumn{1}{l}{Number of observations} & $328$ & $328$ & $328$ &  & $301$
& $301$ & $301$ &  & $325$ & $325$ & $325$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: ``Euclid,'' ``correl,'' and ``min-c'' denote Euclidean, correlation, and min-complement distances, respectively. The LHS variables are as of 2005 or the latest years available in Compustat. The RHS variables are based on our topological characterization of the patent statistics between 1976 and 2005. Standard errors are in parentheses.}
\end{minipage}
\end{center}
\label{Table - Regressions (alt-dist)}
\end{table}

==> Tables/Table_Revenue_n15.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares $\left( n=15\right) $}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.596$ & $0.662$ & $-$ & $-$ &  & $1.586$
& $0.404$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.184)$ & $(0.222)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.178)$ & $(0.214)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $3.233$ & $1.494$ & $-$ & $-$ &  & $%
2.890$ & $0.874$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.866)$ & $(0.849)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.449)$ & $(0.471)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.283$ & $1.585$ & $-$ & $-$ &  & $3.940$
& $1.305$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.574)$ & $(0.593)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.655)$ & $(0.669)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.196$ & $0.601$ &  & $-$
& $-$ & $1.213$ & $0.385$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.211)$ & 
$(0.231)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.195)$ & $(0.218)
$ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.641$ & $0.651$ &  & $-$
& $-$ & $2.332$ & $0.757$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.342)$ & 
$(0.376)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.288)$ & $(0.353)
$ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.040$ & $0.925$ &  & $-$
& $-$ & $2.249$ & $0.650$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.495)$ & 
$(0.517)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.712)$ & $(0.700)
$ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.954$ & $1.792$ &  & $-$
& $-$ & $2.485$ & $0.651$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.732)$ & 
$(0.732)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.585)$ & $(0.605)
$ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $3.336$ & $1.992$ &  & $-$
& $-$ & $2.615$ & $1.015$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.601)$ & 
$(0.627)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.001)$ & $(0.957)
$ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $2.919$ & $1.527$ &  & $-$
& $-$ & $3.471$ & $1.321$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.843)$ & 
$(0.846)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.820)$ & $(0.822)
$ \\ 
\multicolumn{1}{l}{Flare length = 7} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $3.467$ & $1.226$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $(1.411)$ & $(1.348)$ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $4.232$ & $2.424$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.451)$ & 
$(1.426)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.379$ & $1.882$ &  & $-$
& $-$ & $3.843$ & $1.557$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.451)$ & 
$(1.413)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.001)$ & $(0.986)
$ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.327$ & $1.843$ &  & $-
$ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.451)$ & 
$(1.413)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.283$ & $1.827$
&  & $-$ & $-$ & $3.940$ & $1.524$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.558)$ & 
$(0.599)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.639)$ & $(0.690)
$ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.312$ & $-$ & $0.268$ &  & $-$ & $%
0.497$ & $-$ & $0.456$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $(0.047)$ & $\left( -\right) $ & 
$(0.051)$ &  & $\left( -\right) $ & $(0.060)$ & $\left( -\right) $ & $(0.067)
$ \\ 
\multicolumn{1}{l}{Constant} & $7.188$ & $5.850$ & $7.188$ & $6.040$ &  & $%
7.100$ & $4.622$ & $7.100$ & $4.827$ \\ 
\multicolumn{1}{l}{} & $(0.114)$ & $(0.229)$ & $(0.111)$ & $(0.241)$ &  & $%
(0.114)$ & $(0.316)$ & $(0.111)$ & $(0.348)$ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.266$ & $0.362$ & $0.305$ & $0.367$
&  & $0.306$ & $0.440$ & $0.340$ & $0.433$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: The RHS variables are based on the topological characterization of patent statistics between 1976 and 2005. Standard errors are in parentheses.}
\end{minipage}
\end{center}
\label{Table - Revenue (n = 15)}
\end{table}


==> Tables/Table_Revenue_n15_with_sector_dummies.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares $\left( n=15\right) $}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.778$ & $0.901$ & $-$ & $-$ &  & $1.708$
& $0.528$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.172\right) $ & $\left( 0.206\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.168\right) $ & $\left(
0.203\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $3.609$ & $1.924$ & $-$ & $-$ &  & $%
2.969$ & $0.940$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.832\right) $ & $\left( 0.813\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.412\right) $ & $\left(
0.436\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.181$ & $1.601$ & $-$ & $-$ &  & $4.200$
& $1.489$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.534\right) $ & $\left( 0.549\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.597\right) $ & $\left(
0.617\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.374$ & $0.842$ &  & $-$
& $-$ & $1.374$ & $0.533$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.190\right) $ & $\left( 0.209\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.178\right) $ & $\left( 0.204\right) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.978$ & $1.080$ &  & $-$
& $-$ & $2.478$ & $0.951$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.312\right) $ & $\left( 0.346\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.267\right) $ & $\left( 0.329\right) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $1.979$ & $0.967$ &  & $-$
& $-$ & $2.679$ & $1.076$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.461\right) $ & $\left( 0.483\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.667\right) $ & $\left( 0.656\right) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $3.617$ & $2.537$ &  & $-$
& $-$ & $2.701$ & $0.891$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.652\right) $ & $\left( 0.658\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.528\right) $ & $\left( 0.551\right) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.907$ & $1.679$ &  & $-$
& $-$ & $1.780$ & $0.187$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.585\right) $ & $\left( 0.608\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.905\right) $ & $\left( 0.864\right) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.499$ & $2.219$ &  & $-$
& $-$ & $3.289$ & $1.133$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.749\right) $ & $\left( 0.758\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.895\right) $ & $\left( 0.880\right) $ \\ 
\multicolumn{1}{l}{Flare length = 7} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $4.322$ & $2.119$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $\left( 1.256\right) $ & $\left( 1.200\right) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $5.145$ & $3.492$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.288\right) $ & $\left( 1.272\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $4.292$ & $2.912$ &  & $-$
& $-$ & $4.698$ & $2.453$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.288\right) $ & $\left( 1.260\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.895\right) $ & $\left( 0.885\right) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $4.239$ & $2.872$ &  & $-
$ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.288\right) $ & $\left( 1.259\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.183$ & $1.880$
&  & $-$ & $-$ & $4.128$ & $1.750$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.511\right) $ & $\left( 0.550\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.574\right) $ & $\left( 0.629\right) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.288$ & $-$ & $0.235$ &  & $-$ & $%
0.480$ & $-$ & $0.429$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( 0.043\right) $ & $\left(
-\right) $ & $\left( 0.046\right) $ &  & $\left( -\right) $ & $\left(
0.056\right) $ & $\left( -\right) $ & $\left( 0.061\right) $ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.406$ & $0.488$ & $0.457$ & $0.504$
&  & $0.439$ & $0.557$ & $0.481$ & $0.559$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: Standard errors are in parentheses. S\&P economic sector dummies are included.}
\end{minipage}
\end{center}
\label{Table - Revenue (n = 15)}
\end{table}


==> Tables/Table_Revenue_n20_cor.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares $\left( n=20\right) $}
\label{Table - Revenue (n = 20)}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.525$ & $0.518$ & $-$ & $-$ &  & $1.827$
& $0.391$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.183\right) $ & $\left( 0.238\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.184\right) $ & $\left(
0.249\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.338$ & $0.881$ & $-$ & $-$ &  & $%
2.435$ & $0.354$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.442\right) $ & $\left( 0.479\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.397\right) $ & $\left(
0.450\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.885$ & $2.053$ & $-$ & $-$ &  & $3.278$
& $1.009$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.614\right) $ & $\left( 0.651\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.649\right) $ & $\left(
0.659\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.173$ & $0.471$ &  & $-$
& $-$ & $1.403$ & $0.371$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.198\right) $ & $\left( 0.241\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.206\right) $ & $\left( 0.253\right) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.865$ & $0.908$ &  & $-$
& $-$ & $1.920$ & $0.496$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.413\right) $ & $\left( 0.445\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.382\right) $ & $\left( 0.424\right) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $1.857$ & $0.749$ &  & $-$
& $-$ & $2.056$ & $0.614$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.519\right) $ & $\left( 0.551\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.498\right) $ & $\left( 0.520\right) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.198$ & $1.049$ &  & $-$
& $-$ & $3.133$ & $1.238$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.519\right) $ & $\left( 0.554\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.471\right) $ & $\left( 0.534\right) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $3.011$ & $1.742$ &  & $-$
& $-$ & $2.718$ & $0.931$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.650\right) $ & $\left( 0.680\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.471\right) $ & $\left( 0.525\right) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.171$ & $1.814$ &  & $-$
& $-$ & $3.522$ & $1.563$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.553\right) $ & $\left( 0.603\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.696\right) $ & $\left( 0.723\right) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$
& $-$ & $2.429$ & $0.262$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 1.381\right) $ & $\left( 1.339\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.610$ & $2.254$ &  & $-$
& $-$ & $5.508$ & $3.500$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.436\right) $ & $\left( 1.411\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 1.381\right) $ & $\left( 1.333\right) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.370$ & $1.825$ &  & $%
- $ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.018\right) $ & $\left( 1.032\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.885$ & $2.377$
&  & $-$ & $-$ & $3.278$ & $1.329$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.595\right) $ & $\left( 0.654\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.625\right) $ & $\left( 0.662\right) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.315$ & $-$ & $0.259$ &  & $-$ & $%
0.517$ & $-$ & $0.444$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( 0.052\right) $ & $\left(
-\right) $ & $\left( 0.054\right) $ &  & $\left( -\right) $ & $\left(
0.067\right) $ & $\left( -\right) $ & $\left( 0.071\right) $ \\ 
\multicolumn{1}{l}{Constant} & $7.133$ & $5.856$ & $7.133$ & $6.082$ &  & $%
7.136$ & $4.553$ & $7.136$ & $4.916$ \\ 
\multicolumn{1}{l}{} & $\left( 0.117\right) $ & $\left( 0.236\right) $ & $%
\left( 0.114\right) $ & $\left( 0.246\right) $ &  & $\left( 0.108\right) $ & 
$\left( 0.347\right) $ & $\left( 0.104\right) $ & $\left( 0.366\right) $ \\ 
\hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.277$ & $0.359$ & $0.320$ & $0.370$
&  & $0.316$ & $0.434$ & $0.366$ & $0.444$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: The RHS variables are based on the topological characterization of patent statistics between 1976 and 2005. Standard errors are in parentheses.}
\end{minipage}
\end{center}
\end{table}



==> Tables/Table_Revenue_n20_cor_with_sector_dummies.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares $\left( n=20\right) $}
\label{Table - Revenue (n = 20)}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.584$ & $0.571$ & $-$ & $-$ &  & $1.870$
& $0.434$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.174\right) $ & $\left( 0.222\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.172\right) $ & $\left(
0.227\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.483$ & $0.996$ & $-$ & $-$ &  & $%
2.386$ & $0.265$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.418\right) $ & $\left( 0.448\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.375\right) $ & $\left(
0.416\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.724$ & $1.828$ & $-$ & $-$ &  & $3.479$
& $1.194$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.624\right) $ & $\left( 0.645\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.594\right) $ & $\left(
0.593\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.225$ & $0.538$ &  & $-$
& $-$ & $1.440$ & $0.403$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.182\right) $ & $\left( 0.221\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.190\right) $ & $\left( 0.231\right) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $2.145$ & $1.210$ &  & $-$
& $-$ & $2.141$ & $0.703$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.382\right) $ & $\left( 0.409\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.354\right) $ & $\left( 0.387\right) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.287$ & $1.167$ &  & $-$
& $-$ & $2.242$ & $0.790$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.476\right) $ & $\left( 0.507\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.462\right) $ & $\left( 0.476\right) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.082$ & $0.897$ &  & $-$
& $-$ & $3.225$ & $1.246$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.487\right) $ & $\left( 0.522\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.438\right) $ & $\left( 0.495\right) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.960$ & $1.674$ &  & $-$
& $-$ & $2.586$ & $0.716$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.614\right) $ & $\left( 0.640\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.441\right) $ & $\left( 0.489\right) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.632$ & $2.258$ &  & $-$
& $-$ & $3.757$ & $1.746$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.523\right) $ & $\left( 0.570\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.637\right) $ & $\left( 0.656\right) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $3.143$ & $0.939$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $\left( 1.258\right) $ & $\left( 1.205\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.485$ & $2.036$ &  & $-$
& $-$ & $3.722$ & $1.722$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.343\right) $ & $\left( 1.317\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 1.299\right) $ & $\left( 1.234\right) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.700$ & $2.160$ &  & $-
$ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.927\right) $ & $\left( 0.938\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.780$ & $2.258$
&  & $-$ & $-$ & $3.511$ & $1.523$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.595\right) $ & $\left( 0.646\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.571\right) $ & $\left( 0.600\right) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.316$ & $-$ & $0.252$ &  & $-$ & $%
0.516$ & $-$ & $0.446$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( 0.047\right) $ & $\left(
-\right) $ & $\left( 0.050\right) $ &  & $\left( -\right) $ & $\left(
0.060\right) $ & $\left( -\right) $ & $\left( 0.065\right) $ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.384$ & $0.469$ & $0.440$ & $0.487$
&  & $0.434$ & $0.551$ & $0.478$ & $0.555$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: Standard errors are in parentheses. S\&P economic sector dummies are included. See Appendix C for additional results with (i) EBIT, (ii) market capitalization, (iii) $n=15$, (iv) $n=25$, and (v) Euclidean distance.}
\end{minipage}
\end{center}
\end{table}



==> Tables/Table_Revenue_n20_euc.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares ($n=20$, Euclidean Distance)}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.554$ & $0.419$ & $-$ & $-$ &  & $1.658$
& $0.149$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.189)$ & $(0.247)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.182)$ & $(0.241)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.671$ & $1.081$ & $-$ & $-$ &  & $%
2.631$ & $0.388$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.542)$ & $(0.560)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.394)$ & $(0.440)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.745$ & $1.802$ & $-$ & $-$ &  & $3.934$
& $0.972$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.758)$ & $(0.765)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(1.039)$ & $(0.993)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.107$ & $0.321$ &  & $-$
& $-$ & $1.222$ & $0.128$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.220)$ & 
$(0.256)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.204)$ & $(0.246)
$ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.518$ & $0.449$ &  & $-$
& $-$ & $2.126$ & $0.467$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.380)$ & 
$(0.413)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.329)$ & $(0.387)
$ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.094$ & $0.837$ &  & $-$
& $-$ & $2.048$ & $0.404$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.434)$ & 
$(0.475)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.485)$ & $(0.508)
$ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.984$ & $1.555$ &  & $-$
& $-$ & $3.252$ & $1.005$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.604)$ & 
$(0.634)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.485)$ & $(0.554)
$ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.879$ & $1.627$ &  & $-$
& $-$ & $2.796$ & $0.700$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.604)$ & 
$(0.621)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.513)$ & $(0.563)
$ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $2.821$ & $1.202$ &  & $-$
& $-$ & $3.042$ & $0.801$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.035)$ & 
$(1.031)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.826)$ & $(0.829)
$ \\ 
\multicolumn{1}{l}{Flare length = 7} & $-$ & $-$ & $3.642$ & $2.076$ &  & $-$
& $-$ & $2.888$ & $0.416$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.847)$ & 
$(0.858)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.009)$ & $(0.998)
$ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $2.445$ & $-0.059$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $(1.422)$ & $(1.364)$ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.498$ & $2.044$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.459)$ & 
$(1.416)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.246$ & $1.530$ &  & $-
$ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.459)$ & 
$(1.427)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.745$ & $2.084$
&  & $-$ & $-$ & $3.934$ & $1.253$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.736)$ & 
$(0.766)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.009)$ & $(1.010)
$ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.338$ & $-$ & $0.289$ &  & $-$ & $%
0.558$ & $-$ & $0.505$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $(0.051)$ & $\left( -\right) $ & 
$(0.054)$ &  & $\left( -\right) $ & $(0.066)$ & $\left( -\right) $ & $(0.073)
$ \\ 
\multicolumn{1}{l}{Constant} & $7.245$ & $5.811$ & $7.245$ & $6.019$ &  & $%
7.121$ & $4.382$ & $7.121$ & $4.641$ \\ 
\multicolumn{1}{l}{} & $(0.113)$ & $(0.242)$ & $(0.109)$ & $(0.251)$ &  & $%
(0.114)$ & $(0.338)$ & $(0.110)$ & $(0.372)$ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.254$ & $0.352$ & $0.297$ & $0.362$
&  & $0.287$ & $0.430$ & $0.329$ & $0.426$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: The RHS variables are based on the topological characterization of patent statistics between 1976 and 2005. Standard errors are in parentheses.}
\end{minipage}
\end{center}
\label{Table - Revenue (Euclid)}
\end{table}


==> Tables/Table_Revenue_n20_euc_with_sector_dummies.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares ($n=20$, Euclidean Distance)}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.666$ & $0.568$ & $-$ & $-$ &  & $1.720$
& $0.189$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.180\right) $ & $\left( 0.230\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.173\right) $ & $\left(
0.222\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.479$ & $0.946$ & $-$ & $-$ &  & $%
2.646$ & $0.356$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.509\right) $ & $\left( 0.521\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.370\right) $ & $\left(
0.403\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.786$ & $1.878$ & $-$ & $-$ &  & $4.023$
& $0.800$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.699\right) $ & $\left( 0.703\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 1.050\right) $ & $\left(
0.976\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.138$ & $0.410$ &  & $-$
& $-$ & $1.296$ & $0.167$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.206\right) $ & $\left( 0.238\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.193\right) $ & $\left( 0.227\right) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.962$ & $0.913$ &  & $-$
& $-$ & $2.189$ & $0.468$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.355\right) $ & $\left( 0.389\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.306\right) $ & $\left( 0.355\right) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.626$ & $1.427$ &  & $-$
& $-$ & $2.344$ & $0.639$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.401\right) $ & $\left( 0.441\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.447\right) $ & $\left( 0.461\right) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $2.720$ & $1.317$ &  & $-$
& $-$ & $2.984$ & $0.555$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.574\right) $ & $\left( 0.604\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.485\right) $ & $\left( 0.540\right) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.576$ & $1.448$ &  & $-$
& $-$ & $2.652$ & $0.426$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.621\right) $ & $\left( 0.626\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.477\right) $ & $\left( 0.519\right) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $3.615$ & $2.064$ &  & $-$
& $-$ & $3.414$ & $1.038$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.946\right) $ & $\left( 0.943\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.765\right) $ & $\left( 0.758\right) $ \\ 
\multicolumn{1}{l}{Flare length = 7} & $-$ & $-$ & $3.557$ & $2.035$ &  & $-$
& $-$ & $3.623$ & $1.048$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.946\right) $ & $\left( 0.942\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.930\right) $ & $\left( 0.905\right) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $3.180$ & $0.572$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $\left( 1.306\right) $ & $\left( 1.230\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.318$ & $1.868$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.365\right) $ & $\left( 1.325\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 10} & $-$ & $-$ & $3.150$ & $1.505$ &  & $-
$ & $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.329\right) $ & $\left( 1.299\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.850$ & $2.246$
&  & $-$ & $-$ & $4.216$ & $1.085$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.674\right) $ & $\left( 0.705\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 1.018\right) $ & $\left( 1.006\right) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.325$ & $-$ & $0.268$ &  & $-$ & $%
0.561$ & $-$ & $0.517$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( 0.047\right) $ & $\left(
-\right) $ & $\left( 0.049\right) $ &  & $\left( -\right) $ & $\left(
0.059\right) $ & $\left( -\right) $ & $\left( 0.067\right) $ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.376$ & $0.467$ & $0.422$ & $0.478$
&  & $0.398$ & $0.544$ & $0.438$ & $0.539$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: Standard errors are in parentheses. S\&P economic sector dummies are included.}
\end{minipage}
\end{center}
\label{Table - Revenue (Euclid)}
\end{table}


==> Tables/Table_Revenue_n25.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares $\left( n=25\right) $}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.463$ & $0.524$ & $-$ & $-$ &  & $1.333$
& $0.050$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.187)$ & $(0.224)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.184)$ & $(0.209)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.560$ & $1.004$ & $-$ & $-$ &  & $%
2.856$ & $0.499$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.383)$ & $(0.426)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(0.373)$ & $(0.409)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $3.110$ & $1.501$ & $-$ & $-$ &  & $3.932$
& $1.051$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $(0.680)$ & $(0.678)$ & $\left( -\right) $ & $\left(
-\right) $ &  & $(1.065)$ & $(0.976)$ & $\left( -\right) $ & $\left(
-\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.028$ & $0.444$ &  & $-$
& $-$ & $0.919$ & $0.023$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.205)$ & 
$(0.227)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.201)$ & $(0.213)
$ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.740$ & $0.742$ &  & $-$
& $-$ & $1.756$ & $0.172$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.369)$ & 
$(0.404)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.331)$ & $(0.359)
$ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.693$ & $1.448$ &  & $-$
& $-$ & $2.854$ & $0.764$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.391)$ & 
$(0.446)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.361)$ & $(0.419)
$ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $3.040$ & $1.773$ &  & $-$
& $-$ & $2.442$ & $0.565$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.601)$ & 
$(0.626)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.603)$ & $(0.593)
$ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $1.876$ & $0.681$ &  & $-$
& $-$ & $2.979$ & $0.575$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.731)$ & 
$(0.738)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.603)$ & $(0.623)
$ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $2.319$ & $1.126$ &  & $-$
& $-$ & $2.397$ & $0.091$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.601)$ & 
$(0.621)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(0.734)$ & $(0.723)
$ \\ 
\multicolumn{1}{l}{Flare length = 7} & $-$ & $-$ & $3.506$ & $2.106$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.731)$ & 
$(0.752)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $3.385$ & $1.863$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.449)$ & 
$(1.419)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $2.373$ & $0.891$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(1.449)$ & 
$(1.417)$ &  & $\left( -\right) $ & $\left( -\right) $ & $\left( -\right) $
& $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 11} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& 2.874 & 0.283 \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $(1.031)$ & $(0.986)$ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $3.110$ & $1.789$
&  & $-$ & $-$ & $3.932$ & $1.229$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $(0.656)$ & 
$(0.679)$ &  & $\left( -\right) $ & $\left( -\right) $ & $(1.031)$ & $(0.991)
$ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.324$ & $-$ & $0.266$ &  & $-$ & $%
0.564$ & $-$ & $0.529$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $(0.049)$ & $\left( -\right) $ & 
$(0.052)$ &  & $\left( -\right) $ & $(0.059)$ & $\left( -\right) $ & $(0.066)
$ \\ 
\multicolumn{1}{l}{Constant} & $7.130$ & $5.795$ & $7.130$ & $6.034$ &  & $%
7.134$ & $4.365$ & $7.134$ & $4.536$ \\ 
\multicolumn{1}{l}{} & $(0.121)$ & $(0.229)$ & $(0.116)$ & $(0.242)$ &  & $%
(0.123)$ & $(0.310)$ & $(0.119)$ & $(0.343)$ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.256$ & $0.355$ & $0.307$ & $0.365$
&  & $0.253$ & $0.432$ & $0.300$ & $0.428$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: The RHS variables are based on the topological characterization of patent statistics between 1976 and 2005. Standard errors are in parentheses.}
\end{minipage}
\end{center}
\label{Table - Revenue (n = 25)}
\end{table}


==> Tables/Table_Revenue_n25_with_sector_dummies.tex <==

\begin{table}[tbh!!!!]
\caption{Revenues and Flares $\left( n=25\right) $}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccccc}
\hline \hline
LHS variable: & \multicolumn{9}{c}{Log(Revenue in 2005)} \\ \cline{2-10}
Patents acquired by: & \multicolumn{4}{c}{In-house R\&D only} &  & 
\multicolumn{4}{c}{Both R\&D and M\&A} \\ \cline{2-5}\cline{7-10}
& (1) & (2) & (3) & (4) &  & (5) & (6) & (7) & (8) \\ \hline
\multicolumn{1}{l}{Flares only} & $1.497$ & $0.588$ & $-$ & $-$ &  & $1.421$
& $0.096$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.175\right) $ & $\left( 0.206\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.175\right) $ & $\left(
0.191\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flares and islands} & $2.775$ & $1.263$ & $-$ & $-$ &  & $%
2.639$ & $0.216$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.359\right) $ & $\left( 0.394\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 0.369\right) $ & $\left(
0.381\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Islands only} & $2.895$ & $1.268$ & $-$ & $-$ &  & $3.712$
& $0.635$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( 0.655\right) $ & $\left( 0.646\right) $ & $%
\left( -\right) $ & $\left( -\right) $ &  & $\left( 1.008\right) $ & $\left(
0.891\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 1} & $-$ & $-$ & $1.131$ & $0.537$ &  & $-$
& $-$ & $0.968$ & $0.073$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.192\right) $ & $\left( 0.211\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.187\right) $ & $\left( 0.194\right) $ \\ 
\multicolumn{1}{l}{Flare length = 2} & $-$ & $-$ & $1.769$ & $0.793$ &  & $-$
& $-$ & $1.898$ & $0.278$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.343\right) $ & $\left( 0.369\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.316\right) $ & $\left( 0.334\right) $ \\ 
\multicolumn{1}{l}{Flare length = 3} & $-$ & $-$ & $2.741$ & $1.470$ &  & $-$
& $-$ & $2.880$ & $0.732$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.378\right) $ & $\left( 0.425\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.349\right) $ & $\left( 0.393\right) $ \\ 
\multicolumn{1}{l}{Flare length = 4} & $-$ & $-$ & $3.067$ & $1.719$ &  & $-$
& $-$ & $2.429$ & $0.539$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.565\right) $ & $\left( 0.588\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.571\right) $ & $\left( 0.548\right) $ \\ 
\multicolumn{1}{l}{Flare length = 5} & $-$ & $-$ & $2.390$ & $1.163$ &  & $-$
& $-$ & $2.789$ & $0.296$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.677\right) $ & $\left( 0.678\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.566\right) $ & $\left( 0.575\right) $ \\ 
\multicolumn{1}{l}{Flare length = 6} & $-$ & $-$ & $2.127$ & $0.882$ &  & $-$
& $-$ & $2.691$ & $0.267$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.566\right) $ & $\left( 0.581\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.679\right) $ & $\left( 0.659\right) $ \\ 
\multicolumn{1}{l}{Flare length = 7} & $-$ & $-$ & $3.289$ & $1.862$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.777\right) $ & $\left( 0.780\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 8} & $-$ & $-$ & $4.082$ & $2.543$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.336\right) $ & $\left( 1.297\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 9} & $-$ & $-$ & $3.070$ & $1.571$ &  & $-$
& $-$ & $-$ & $-$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
1.336\right) $ & $\left( 1.295\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ & $\left( -\right) $ \\ 
\multicolumn{1}{l}{Flare length = 11} & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$
& $3.590$ & $0.944$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
-\right) $ & $\left( -\right) $ &  & $\left( -\right) $ & $\left( -\right) $
& $\left( 0.959\right) $ & $\left( 0.893\right) $ \\ 
\multicolumn{1}{l}{Flare length = $\infty $} & $-$ & $-$ & $2.966$ & $1.549$
&  & $-$ & $-$ & $3.806$ & $0.916$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( -\right) $ & $\left(
0.637\right) $ & $\left( 0.656\right) $ &  & $\left( -\right) $ & $\left(
-\right) $ & $\left( 0.959\right) $ & $\left( 0.908\right) $ \\ 
\multicolumn{1}{l}{Log(Patents)} & $-$ & $0.315$ & $-$ & $0.269$ &  & $-$ & $%
0.581$ & $-$ & $0.534$ \\ 
\multicolumn{1}{l}{} & $\left( -\right) $ & $\left( 0.045\right) $ & $\left(
-\right) $ & $\left( 0.048\right) $ &  & $\left( -\right) $ & $\left(
0.054\right) $ & $\left( -\right) $ & $\left( 0.061\right) $ \\ \hline
\multicolumn{1}{l}{Adjusted $R^{2}$} & $0.378$ & $0.472$ & $0.415$ & $0.475$
&  & $0.349$ & $0.543$ & $0.412$ & $0.541$ \\ 
\multicolumn{1}{l}{Number of observations} & $286$ & $286$ & $286$ & $286$ & 
& $288$ & $288$ & $288$ & $288$ \\ \hline \hline
\end{tabular}
\begin{minipage}{450pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: Standard errors are in parentheses. S\&P economic sector dummies are included.}
\end{minipage}
\end{center}
\label{Table - Revenue (n = 25)}
\end{table}


==> Tables/Table_flares.tex <==

\begin{table}[tbh!!!!]
\caption{Firm Count by Flare Type and Length}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{cccccccc}
\hline \hline
Patents acquired by: & \multicolumn{3}{c}{In-house R\&D only} &  & 
\multicolumn{3}{c}{Both R\&D and M\&A} \\ \cline{2-4}\cline{6-8}
KeplerMapper resolution: & $n=15$ & $n=20$ & $n=25$ &  & $n=15$ & $n=20$ & $n=25$
\\ 
& $\left( 1\right) $ & $\left( 2\right) $ & $\left( 3\right) $ &  & $\left(
4\right) $ & $\left( 5\right) $ & $\left( 6\right) $ \\ \hline
\multicolumn{1}{l}{Type} &  &  &  &  &  &  &  \\ 
\multicolumn{1}{l}{0: No flares} & $211$ & $200$ & $196$ &  & $199$ & $218$
& $187$ \\ 
\multicolumn{1}{l}{1: Flares only} & $112$ & $114$ & $114$ &  & $117$ & $95$
& $126$ \\ 
\multicolumn{1}{l}{2: Flares and islands} & $3$ & $13$ & $17$ &  & $12$ & $15
$ & $18$ \\ 
\multicolumn{1}{l}{3: Islands only} & $7$ & $6$ & $6$ &  & $5$ & $5$ & $2$
\\ \hline
\multicolumn{1}{l}{Length} &  &  &  &  &  &  &  \\ 
\multicolumn{1}{l}{0 (No flares)} & $211$ & $200$ & $196$ &  & $199$ & $218$
& $187$ \\ 
\multicolumn{1}{l}{1} & $69$ & $83$ & $76$ &  & $82$ & $64$ & $85$ \\ 
\multicolumn{1}{l}{2} & $21$ & $13$ & $18$ &  & $28$ & $14$ & $22$ \\ 
\multicolumn{1}{l}{3} & $9$ & $8$ & $15$ &  & $5$ & $8$ & $19$ \\ 
\multicolumn{1}{l}{4} & $4$ & $8$ & $6$ &  & $6$ & $9$ & $6$ \\ 
\multicolumn{1}{l}{5} & $6$ & $5$ & $4$ &  & $2$ & $9$ & $6$ \\ 
\multicolumn{1}{l}{6} & $3$ & $7$ & $6$ &  & $3$ & $4$ & $4$ \\ 
\multicolumn{1}{l}{7} & $0$ & $0$ & $4$ &  & $1$ & $0$ & $0$ \\ 
\multicolumn{1}{l}{8} & $1$ & $0$ & $1$ &  & $0$ & $1$ & $0$ \\ 
\multicolumn{1}{l}{9} & $1$ & $1$ & $1$ &  & $2$ & $1$ & $0$ \\ 
\multicolumn{1}{l}{10} & $1$ & $2$ & $0$ &  & $0$ & $0$ & $0$ \\ 
\multicolumn{1}{l}{11} & $0$ & $0$ & $0$ &  & $0$ & $0$ & $2$ \\ 
\multicolumn{1}{l}{$\infty $ (Islands only)} & $7$ & $6$ & $6$ &  & $5$ & $5$
& $2$ \\ \hline \hline
\end{tabular}
\begin{minipage}{350pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: The underlying Mapper graphs are based on correlation distance. Column (2) corresponds to Figure \ref{Figure - mapper(n20_m0_cor)} in the introduction. Column (5) corresponds to Figure \ref{Figure - mapper(n20_m2_cor)}.}
\end{minipage}
\end{center}
\label{Table - Flares}
\end{table}


==> Tables/Table_sumstats_by_sector.tex <==
\begin{table}[tbh]
\caption{Patents and Flares by Sector}
\begin{center}
\fontsize{9pt}{11pt}\selectfont%
\begin{tabular}{lcccccccccc}
\hline \hline
& \multicolumn{3}{c}{Patent count (mean)} &  & \multicolumn{6}{c}{Flare type
(\# firms)} \\ \cline{2-4}\cline{6-11}
& R\&D & M\&A & Total &  & No & Flares & Flares \& & Islands & Total & \%
flares \\ 
S\&P economic sector &  &  &  &  & flares & only & islands & only &  &  \\ 
\hline
Technology & $2,665$ & $339$ & $3,004$ &  & $60$ & $37$ & $7$ & $2$ & $106$
& $43.4$ \\ 
Capital goods & $1,836$ & $241$ & $2,077$ &  & $65$ & $21$ & $2$ & $3$ & $91$
& $28.6$ \\ 
Health care & $890$ & $248$ & $1,138$ &  & $33$ & $11$ & $0$ & $0$ & $44$ & $%
25.0$ \\ 
Consumer cyclicals & $453$ & $41$ & $494$ &  & $22$ & $6$ & $0$ & $0$ & $28$
& $21.4$ \\ 
Basic materials & $2,389$ & $239$ & $2,628$ &  & $13$ & $9$ & $1$ & $0$ & $23
$ & $43.5$ \\ 
Consumer staples & $1,406$ & $212$ & $1,617$ &  & $10$ & $2$ & $2$ & $0$ & $%
14$ & $28.6$ \\ 
Energy & $2,803$ & $694$ & $3,497$ &  & $1$ & $2$ & $1$ & $0$ & $4$ & $75.0$
\\ 
Communication services & $5,456$ & $43$ & $5,500$ &  & $0$ & $2$ & $1$ & $0$
& $3$ & $100.0$ \\ 
Transportation & $13,500$ & $40$ & $13,540$ &  & $0$ & $1$ & $0$ & $0$ & $1$
& $100.0$ \\ 
Utilities & $711$ & $243$ & $954$ &  & $0$ & $1$ & $0$ & $0$ & $1$ & $100.0$
\\ 
No S\&P sector & $297$ & $259$ & $556$ &  & $14$ & $3$ & $1$ & $0$ & $18$ & $%
22.2$ \\ \hline \hline
\end{tabular}
\begin{minipage}{475pt}
{\fontsize{9pt}{9pt}\selectfont \smallskip  \textit{Note}: ``No S\&P sector'' means the firm does not have an S\&P economic sector designation. Flare types and lengths are based on Figure \ref{Figure - mapper(n20_m2_cor)} (i.e., the Mapper graph of both R\&D and M\&A patents with $n=20$ and correlation distance).}
\end{minipage}
\end{center}
\label{Table - Sumstats by sector}
\end{table}

